Dropping Pixels for Adversarial Robustness

Deep neural networks are vulnerable against adversarial examples. In this paper, we propose to train and test the networks with randomly subsampled images with high drop rates. We show that this approach significantly improves robustness against adversarial examples in all cases of bounded L0, L2 and L_inf perturbations, while reducing the standard accuracy by a small value. We argue that subsampling pixels can be thought to provide a set of robust features for the input image and, thus, improves robustness without performing adversarial training.

==> Analysis.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.9\linewidth]{Figures/expand.pdf}
	\caption{\small Expanding and random dropping for defending against adversarial examples.}
	\label{fig:expand}
\end{figure}


\subsubsection{Analysis}

We show that random subsampling of correlated features improves robustness against adversarial examples with bounded $L_2$ perturbations. 
Specifically, we prove that introducing redundancy to inputs with uncorrelated features and then randomly dropping features reduces attack effectiveness. 
The intuition is that the adversary needs to distribute their budget to all features in such a way that the expected attack success rate is maximized. This, however, reduces the attack effectiveness compared to the case that the attacker knows the exact sampling pattern. 


Let $F: x\rightarrow y$ be a function that takes the input $x\in \mathbb{R}^d$ and outputs the label $y\in \mathbb{R}$. We expand the input to vector $z \in\mathbb{R}^D, D>d,$ as $z=Ax$, where $A\in\mathbb{R}^{D\times d}$ is a matrix of rank $d$, i.e., all of its $d\times d$ submatrices are invertible. 
We then replace a random subset of $z$ with $D-d$ elements with zero and recover $x$ from the remaining $d$ elements. 
This is possible because any subset of $D-d$ elements of vector $z$ can be obtained from the other $d$ elements. Figure~\ref{fig:expand} shows the problem model. 


Let $S$ be a random subset of size $d$ of the set $\{0,\cdots,D-1\}$, and $M$ be a diagonal matrix of size $D\times D$, in which $M_{i,i}=1$, for $i\in S$, and zero otherwise. 
%We construct the vector $z_S=Mz$. 
We write $A_S = MA$ and $B_S={A_S}^+$, where ${A_S}^+$ denotes the pseudo-inverse of ${A_S}$. We have $x=B_S z$. 


The adversary is allowed to perturb $z$ to $z'=z+\Delta z$ such that $\|\Delta z\|_2^2\leq\epsilon$. The corresponding perturbed input is obtained as $x'=B_S (z+\Delta z)=x+B_S \Delta z$. Thus, $\Delta x=B_S \Delta z$ is the corresponding perturbation added to input. 
Let $\Delta x^*$ be the optimal perturbation to $x$, which is deterministic (not dependent on the sampling) and is known to adversary. 
The adversary's problem is to find $\Delta z$ such that the corresponding $\Delta x$ is most aligned with optimal perturbation $\Delta x^*$. 
The problem is formally stated as follows:
\begin{align}\label{eq:adv} 
\max_{\Delta z} (B_S \Delta z)^T \Delta x^*,  \mbox{ s.t. } \|\Delta z\|_2^2\leq\epsilon. 
\end{align}

\vspace{0.1cm}
\noindent{\bf Lemma 1.} 
{\it The optimal solution to problem~\ref{eq:adv} is $\Delta z^*=\frac{1}{\lambda}B_S^T \Delta x^*$, where $\lambda=\frac{1}{\sqrt{\epsilon}}\|B_S^T \Delta x^*\|_2$. 

\vspace{0.1cm}
\noindent{\bf Proof.}
We use standard Lagrangian multiplier method. Let $f = (B_S \Delta z)^T \Delta x^* - \frac{\lambda}{2} \|\epsilon-\Delta z\|_2^2.$ 
By setting $\nabla_{\Delta z}f=B_S^T \Delta x^*-\lambda \Delta z=0$, we obtain $\Delta z^*=\frac{1}{\lambda}B_S^T \Delta x^*$. 
Clearly, we have $\|\Delta z^*\|_2^2=\epsilon$, which can be used to obtain $\lambda$}. $\blacksquare$

\vspace{0.1cm}

The adversary, however, does not know the sampling positions and, hence, does not know the matrix $B_S$. 
As a result, $\Delta z$ is generated such that the corresponding perturbation in $x$ is, on average, most aligned with $\Delta x^*$. 
For $\Delta z$, the average perturbation in $x$ is obtained as $\bar{\Delta x}=\mathbb{E}_S[B_S] \Delta z$. 
%Let $B=\mathbb{E}_S[B_S]$. 
Thus, the adversary's problem in random sampling case is as follows:
\begin{align}\label{eq:adv2} 
\max_{\Delta z} (\mathbb{E}_S[B_S] \Delta z)^T \Delta x^*,  \mbox{ s.t. } \|\Delta z\|_2^2\leq\epsilon. 
\end{align}


\vspace{0.1cm}
\noindent{\bf Theorem:} 
{\it Let $\Delta x=B_S \Delta z$. }

\vspace{0.1cm}

\noindent{\bf Proof.} 
Let ${\Delta x}_1 = \frac{1}{\lambda_1}B_S B_S^T \Delta x^*$, where $\lambda_1=\frac{1}{\sqrt{\epsilon}}\|B_S^T \Delta x^*\|_2$. 
Also let ${\Delta x}_2 = \frac{1}{\lambda_2}B_S \mathbb{E}_S[B]^T \Delta x^*$, where $\lambda_2=\frac{1}{\sqrt{\epsilon}}\|\mathbb{E}_S[B]^T \Delta x^*\|_2$. 
Let ${B_S}_i$ be the $i$-th column of $B_S$. We have ${B_S}_i=\frac{D}{d}{\mathbb{E}_S[B_S]}_i$ if $i\in S$ and zero otherwise. 
Hence, $\mathbb{E}_S[B] \mathbb{E}_S[B]^T = \frac{d}{D}\mathbb{E}_S[B_S B_S^T]$. 
Thus,  
%\begin{align}
%\nonumber\mathbb{E}_S[\lambda_1]&=\frac{1}{\sqrt{\epsilon}}\sqrt{\Delta {x^*}^T\mathbb{E}_S[B_S B_S^T]\Delta x^*} \\
%\nonumber & =\sqrt{\frac{D}{d}} \frac{1}{\sqrt{\epsilon}}\sqrt{\Delta {x^*}^T\mathbb{E}_S[B] \mathbb{E}_S[B]^T\Delta x^*} \\
%\nonumber & =\lambda_2\sqrt{\frac{D}{d}} 
%\end{align}
\begin{align}
\nonumber \lambda_2&=\frac{1}{\sqrt{\epsilon}}\sqrt{\Delta {x^*}^T\mathbb{E}_S[B] \mathbb{E}_S[B]^T\Delta x^*} \\
\nonumber & =\sqrt{\frac{d}{D}} \frac{1}{\sqrt{\epsilon}}\sqrt{\Delta {x^*}^T\mathbb{E}_S[B_S B_S^T]\Delta x^*} \\
\nonumber & = WRONG\mathbb{E}_S[\lambda_1]\sqrt{\frac{d}{D}}.
\end{align}

We have $\mathbb{E}_S[B_S]=\frac{d}{D}B_S + B'$, where $B_S B'^T=0$.

Hence, ${\Delta x}_2 = \frac{d}{D} \frac{1}{\lambda_2}B_S B_S^T \Delta x^*$


%Case 1: $\mathbb{E}_S[B_S B_S^T]$
%
%Case 2: $\mathbb{E}_S[B] \mathbb{E}_S[B]^T$




 




%\begin{align}\label{eq:lag} 
%\min_{\lambda>0}\max_{\Delta z} \hspace{0.1cm} &(B \Delta z)^T \Delta x^* +\lambda (\epsilon-\|\Delta z\|_2^2)
%\end{align}


%We show that with uncertainty over $M$, $E_M[\tilde{\Delta x}^T \Delta x^*]<\|\Delta x^*\|_2^2$. 
%
%
%Since the columns of $A$ are linearly independent, the pseudo-inverse of matrix $A$ is obtained as $A^{+}=(A^{T}A)^{-1}A^{T}$. We have $x=A^{+}z$.
%
%Let $B=\frac{1}{n} \sum_{S\subset \{0,\cdots,D-1\}, |S|=d} B_S$, where $n$ is the number of subsets of size $d$ of the set $\{0,\cdots,D-1\}$ ($D$ choose $d$). 
%Matrix $B$ is the pseudo-inverse of the matrix $A$, i.e., $x=Bz$. 




